A Greedy Sensor Selection Algorithm for Hyperparameterized Linear Bayesian Inverse Problems

We consider optimal sensor placement for a family of linear Bayesian inverse problems characterized by a deterministic hyper-parameter. The hyper-parameter describes distinct configurations in which measurements can be taken of the observed physical system. To optimally reduce the uncertainty in the system's model with a single set of sensors, the initial sensor placement needs to account for the non-linear state changes of all admissible configurations. We address this requirement through an observability coefficient which links the posteriors' uncertainties directly to the choice of sensors. We propose a greedy sensor selection algorithm to iteratively improve the observability coefficient for all configurations through orthogonal matching pursuit. The algorithm allows explicitly correlated noise models even for large sets of candidate sensors, and remains computationally efficient for high-dimensional forward models through model order reduction. We demonstrate our approach on a large-scale geophysical model of the Perth Basin, and provide numerical studies regarding optimality and scalability with regard to classic optimal experimental design utility functions.

==> 004_comments.tex <==
\section*{Comments - draft version only}


Here are some helpful boxes and colors for working on this draft.
We will take them out for the final version.

\myblue{Blue: leave out? Please indicate if you agree or disagree}

\myorange{Orange: in needs of re-wording or better vocabulary for one reason or another. Please provide suggestions.}

\myred{Red: content that is possibly wrong or potentially misleading. Provide input if possible.}

\todo[inline]{todo: generic todo box}
\missing[inline]{missing: box for marking that something is missing}
\idea[inline]{idea: here's another way to do something, is this better, please provide input if you have an opinion}
\change[inline]{change: reminder to change something}
\unsure[inline]{unsure: help needed, something is definitely going wrong here}
\question[inline]{question: A question waiting for your answer}
\info[inline]{info: here's an explanation for a choice made before or after}


\textbf{variable names:}
\begin{itemize}
    \item N: I'm at a bit of a loss as to what to call the three axes for the Perth Basin plot (fig. 1). Figures 9 and 10 use z and y, so ideally I keep it that way. However we are already using x for the state. Maybe we call the state u instead and the parameter m? I called the state x in my thesis for consistency with the other chapters, but there's no reason here to keep it that way. \textbf{At Peng:} What do you think is the most common in the literature?
    \textit{from Peng: I think you can use $x = (x_1, x_2, x_3)$ as the point of location, as it appears in the definition of the sensor locations in page 17. It is also fine to use $(x,y,z)$ but it needs to be consistent. You can either keep using $x_\theta$ as the state variable for simplicity, or use $u$ as the state variable and $m$ as the parameter. A common use for parameter is $\theta$ but it is already used for the hyper-parameter.}
\end{itemize}


